Key-Graph Transformer for Image Restoration

While it is crucial to capture global information for effective image restoration (IR), integrating such cues into transformer-based methods becomes computationally expensive, especially with high input resolution. Furthermore, the self-attention mechanism in transformers is prone to considering unnecessary global cues from unrelated objects or regions, introducing computational inefficiencies. In response to these challenges, we introduce the Key-Graph Transformer (KGT) in this paper. Specifically, KGT views patch features as graph nodes. The proposed Key-Graph Constructor efficiently forms a sparse yet representative Key-Graph by selectively connecting essential nodes instead of all the nodes. Then the proposed Key-Graph Attention is conducted under the guidance of the Key-Graph only among selected nodes with linear computational complexity within each window. Extensive experiments across 6 IR tasks confirm the proposed KGT's state-of-the-art performance, showcasing advancements both quantitatively and qualitatively.

==> tables/sota_comparison.tex <==
\begin{table*}[!t]
	\centering
	\caption{\textcolor{black}{The Performance of the latest state-of-the-art 3D Skeleton-based methods on NTU-RGB+D dataset.}}
	\label{tab:table1}
        \resizebox{1.\textwidth}{!}{
	\begin{tabular}{cccccc}
		\toprule[1pt]
		\multicolumn{6}{c}{\textbf{NTU-RGB+D dataset}}                            \\ 
		Rank & Paper & Year & Accuracy (C-View) & Accuracy (C-Subject) & Method \\ \Xhline{0.8pt}
            1     &Wang \emph{et al}.~\cite{wang20233mformer} & 2023 & 98.7 & 94.8 & Two-stream Transformer \\ 
            2 & Duan \etal ~\cite{duan2022dg} & 2022 & 97.5 & 93.2 & Dynamic group GCN \\ 
            3     &Liu \emph{et al}.~\cite{liu2023temporal} & 2023 & 96.8 & 92.8 & Temporal decoupling GCN\\ 
            4 & Zhou \etal ~\cite{zhou2022hypergraph} & 2022 & 96.5 & 92.9 & Transformer \\ 
            
            5 & Chen \etal ~\cite{chen2021channel} & 2021 & 96.8 & 92.4 & Topology refinement GCN \\ 
            
            6 & Zeng \etal ~\cite{zeng2021learning} & 2021 & 96.7 & 91.6 & Skeletal GCN \\ 

            7 & Liu \etal ~\cite{liu2020disentangling} & 2020 & 96.2 & 91.5 & Disentangling and unifying GCN \\ 

            8 & Ye \etal ~\cite{ye2020dynamic} & 2020 & 96.0 & 91.5 & Dynamic GCN \\ 

		9 & Shi \etal~\cite{shi2019skeleton}        & 2019 &96.1 &89.9 & Directed graph neural networks\\ 
		10 &Shi \emph{et al}.~\cite{shi2019two}             & 2018 &95.1 &88.5 &Two-stream adaptive GCN\\ 
		11    &Zhang \emph{et al}.~\cite{zhang2019view}        & 2018 &95.0 &89.2 &LSTM based RNN        \\ 
		12    &Si \emph{et al}.~\cite{si19atten}               & 2019 &95.0 &89.2 &AGC-LSTM(Joints\&Part)        \\ 
		13    &Hu \emph{et al}.~\cite{hu2019skeleton}          & 2018 &94.9 &89.1 &Non-local S-T + frequency attention    \\ 
		14     &Li \emph{et al}.~\cite{li2019actional}            & 2019 &94.2 &86.8 &GCN        \\ 
		
		15     &Liang \emph{et al}.~\cite{liang2019three}       & 2019 &93.7 &88.6 &3S-CNN + multi-task ensemble learning    \\ 
		
		16     &Song \emph{et al}.~\cite{song2019richlt}        & 2019 &93.5 &85.9 &Richly activated GCN     \\
		17     &Zhang \emph{et al}.~\cite{zhang2019semantics}   & 2019 &93.4 &86.6 &Semantics-guided GCN     \\ 
		18    &Xie \emph{et al}.~\cite{li2021memory}          & 2018 &93.2 &82.7 &RNN+CNN+Attention    \\ \bottomrule[0.1em]     
	\end{tabular}
        }
\end{table*}


\begin{table*}[t]
	\centering
	\caption{\textcolor{black}{The Performance of the latest state-of-the-art 3D Skeleton-based methods on NTU-RGB+D 120 dataset.}}
	\label{tab:table2}
        \resizebox{1.\textwidth}{!}{
	\begin{tabular}{cccccc}
		\toprule[0.1em]    
		\multicolumn{6}{c}{\textbf{NTU-RGB+D 120 dataset}}                        \\ 
		Rank & Paper & Year & Accuracy (C-Subject) & Accuracy (C-Setup) & Method \\ 
		\Xhline{0.8pt}
            1     &Wang \emph{et al}.~\cite{wang20233mformer} & 2023 & 92.0 & 93.8 & Two-stream Transformer \\ 
            2     &Xu \emph{et al}.~\cite{xu2023language} & 2023 & 90.7 & 91.8 & Language Knowledge-Assisted \\

            3     &Zhou \etal \cite{zhou2022hypergraph} & 2022 & 89.9 & 91.3 & Transformer \\ 

            4     &Duan \etal \cite{duan2022dg} & 2022 & 89.6 & 91.3 & Dynamic group GCN \\ 
            
            5     &Chen \etal \cite{chen2021channel} & 2021 & 88.9 & 90.6 & Topology refinement GCN \\ 

            6     &Chen \etal \cite{chen2021learning} & 2021 & 88.2 & 89.3 & Spatial-Temporal GCN \\ 

            7     &Liu \etal \cite{liu2020disentangling} & 2020 & 86.9 & 88.4 & Disentangling and unifying GCN \\ 

            8     &Cheng \etal \cite{cheng2020skeleton} & 2020 & 85.9 & 87.6 & Shift GCN \\ 


		9     &Caetano \emph{et al}.~\cite{caetano2019skeleton}& 2019 &67.9 &62.8 &Tree Structure + CNN    \\ 
		
		10     &Caetano \emph{et al}.~\cite{caetano2019skelemotion}  & 2019 &67.7 &66.9 &SkeleMotion        \\ 
		
		11    &Liu \emph{et al}.~\cite{liu2018recognizing}     & 2018 &64.6 &66.9 &Body Pose Evolution Map        \\ 
		
		12     &Ke \emph{et al}.~\cite{ke2018learning}          & 2018 &62.2 &61.8 &Multi-Task CNN with RotClips        \\ 
		
	      13   &Liu \emph{et al}.~\cite{liu2017skeleton}        & 2017 &61.2 &63.3 &Two-Stream Attention LSTM        \\ 
		
		14     &Liu \emph{et al}.~\cite{liu2017enhanced}        & 2017 &60.3 &63.2 &Skeleton Visualization (Single Stream)        \\ 
		
		15     &Jun \emph{et al}.~\cite{liu2019skeleton}        & 2019 &59.9 &62.4 &Online+Dilated CNN         \\ 
		
		16     &Ke \emph{et al}.~\cite{ke2017new}               & 2017 &58.4 &57.9 &Multi-Task Learning CNN                                         \\ 
		
		17     &Jun \emph{et al}.~\cite{liu2017global}          & 2017 &58.3 &59.2 &Global Context-Aware Attention LSTM        \\ 
		
		18    &Jun \emph{et al}.~\cite{liu2016spatio}          & 2016 &55.7 &57.9 &Spatio-Temporal LSTM        \\ 
		\bottomrule[0.1em]
	\end{tabular}
        }
\end{table*}

